Workflow Discovery from Dialogues in the Low Data Regime

Text-based dialogues are now widely used to solve real-world problems. In cases where solution strategies are already known, they can sometimes be codified into workflows and used to guide humans or artificial agents through the task of helping clients. We introduce a new problem formulation that we call Workflow Discovery (WD) in which we are interested in the situation where a formal workflow may not yet exist. Still, we wish to discover the set of actions that have been taken to resolve a particular problem. We also examine a sequence-to-sequence (Seq2Seq) approach for this novel task. We present experiments where we extract workflows from dialogues in the Action-Based Conversations Dataset (ABCD). Since the ABCD dialogues follow known workflows to guide agents, we can evaluate our ability to extract such workflows using ground truth sequences of actions. We propose and evaluate an approach that conditions models on the set of possible actions, and we show that using this strategy, we can improve WD performance. Our conditioning approach also improves zero-shot and few-shot WD performance when transferring learned models to unseen domains within and across datasets. Further, on ABCD a modified variant of our Seq2Seq method achieves state-of-the-art performance on related but different problems of Action State Tracking (AST) and Cascading Dialogue Success (CDS) across many evaluation metrics.

==> 6_limitations.tex <==
\section*{Limitations}
Due to the text nature of the output in our text-to-text approach, two issues arise during evaluation. First, when evaluating the zero-shot performance, we use the BERTScore to establish if an action was predicted correctly. We chose a high F1-score threshold (i.e., 95\%) for a fair evaluation. However, a high threshold induces false negatives. For example, if the gold value is \emph{offer promo code}, predicting \emph{give promo code} and \emph{offer code} give an F1-score of 96.6\% and 91.1\%, respectively, and with our setup \emph{offer code} is deemed invalid even if it is semantically equivalent. Lowering the threshold can resolve the example described earlier. However, it will increase the false positives. For example, if the gold value is \emph{book restaurant}, predicting \emph{find restaurant} gives an F1-score of 93.4\%, and here the predicted value is not equivalent to the gold one in MultiWOZ. This issue is more prominent in our case since the action names are short. Using longer descriptions might solve this issue. However, it will increase the model target length, reducing the performance. All this makes choosing the threshold a complex balancing act. Second, a similar issue occurs when evaluating the slot values where a model predicts a more refined value (e.g., predicting \emph{cambridge museum of technology} instead of \emph{museum}). While we can handle both cases with more clever evaluation methods, this adds more complexity to the evaluation process on top of the complexity of the task at hand (i.e., WD task). Finally, in all our experimental settings, we showed that using our conditioning technique drastically improves the performance. However, this technique assumes that the possible actions are known, something not always true in a real-world application.

==> 7_ethics.tex <==
\section*{Ethics Statement}
In this work, we set to extract workflows from task-oriented dialogues. To this end, we use large language models to generate the desired workflows in an open-ended manner instead of a simple classification task. These models have been trained in an unsupervised way on a large set of data collected from the web. So, this data may contain bias or stereotypes like race and gender that might manifest during the text output generation. Moreover, the performance might be biased toward the English-speaking population since English is the most prominent language in open source text datasets.

